SF-sketch: A Two-stage Sketch for Data Streams

A sketch is a probabilistic data structure used to record frequencies of items in a multi-set. Sketches are widely used in various fields, especially those that involve processing and storing data streams. In streaming applications with high data rates, a sketch "fills up" very quickly. Thus, its contents are periodically transferred to the remote collector, which is responsible for answering queries. In this paper, we propose a new sketch, called Slim-Fat (SF) sketch, which has a significantly higher accuracy compared to prior art, a much smaller memory footprint, and at the same time achieves the same speed as the best prior sketch. The key idea behind our proposed SF-sketch is to maintain two separate sketches: a small sketch called Slim-subsketch and a large sketch called Fat-subsketch. The Slim-subsketch is periodically transferred to the remote collector for answering queries quickly and accurately. The Fat-subsketch, however, is not transferred to the remote collector because it is used only to assist the Slim-subsketch during the insertions and deletions and is not used to answer queries. We implemented and extensively evaluated SF-sketch along with several prior sketches and compared them side by side. Our experimental results show that SF-sketch outperforms the most widely used CM-sketch by up to 33.1 times in terms of accuracy. We have released the source codes of our proposed sketch as well as existing sketches at Github. The short version of this paper will appear in ICDE 2017.

==> author_format.tex <==
\author{Tong Yang, Gaogang xie, Yanbiao Li, Qiaobin Fu, Alex X. Liu, Qi Li, Laurent Mathy}

\numberofauthors{6}
\author{
\alignauthor
Tong Yang,Gaogang Xie*\\
       %\affaddr{Institute of Computing Technology, Chinese Academy of Sciences (CAS), China.}\\
       \affaddr{ICT, CAS, China.}\\
       \email{yangtongemail@gmail.com, *xie@ict.ac.cn}
\alignauthor
YanBiao Li\\
       %\affaddr{College of Computer Science and Electronic Engineering, Hunan University, China}\\
       \affaddr{Hunan University, China}\\
       \email{lybmath\_cs@hnu.edu.cn}
\alignauthor
Qiaobin Fu\\
       \affaddr{ICT, CAS, China}\\
       \email{fuqiaobin@ict.ac.cn}
\and
\alignauthor Alex X. Liu\\
       \affaddr{Department of Computer Science and Engineering, Michigan State University}\\
       \email{alexliu@cse.msu.edu}
\alignauthor Qi Li\\
       \affaddr{ICT, CAS, China}\\
       \email{liqi19872006@gmail.com}
\alignauthor Laurent Mathy\\
       \affaddr{University of Liege, Belgium}\\
       \email{laurent.mathy@ulg.ac.be}
}


\author{\IEEEauthorblockN{Tong Yang\IEEEauthorrefmark{1},
Xiaoming Li\IEEEauthorrefmark{1},
Alex X. Liu\IEEEauthorrefmark{2},
Qiaobin Fu\IEEEauthorrefmark{3},
Gaogang Xie\IEEEauthorrefmark{4}}
\IEEEauthorblockA{\IEEEauthorrefmark{1}Computer Science Department, Peking University, Beijing, China}
\IEEEauthorblockA{\IEEEauthorrefmark{2}Department of Computer Science and Engineering, Michigan State University}
\IEEEauthorblockA{\IEEEauthorrefmark{3}Computer Science Department, Boston University, USA}
\IEEEauthorblockA{\IEEEauthorrefmark{4}ICT, CAS, China}
}

==> ref.tex <==
\begin{thebibliography}{10}



\bibitem{sdm10sketch}
C.~C. Aggarwal and S.~Y. Philip.
\newblock On classification of high-cardinality data streams.
\newblock In {\em SDM}, volume~10, pages 802--813. SIAM, 2010.


\bibitem{chen2010tracking}
A.~Chen, Y.~Jin, J.~Cao, and L.~E. Li.
\newblock Tracking long duration flows in network traffic.
\newblock In {\em \Proc IEEE INFOCOM}, 2010.

\bibitem{cormode2005sketching}
G.~Cormode and M.~Garofalakis.
\newblock Sketching streams through the net: Distributed approximate query
  tracking.
\newblock In {\em Proceedings of the 31st international conference on Very
  large data bases}, pages 13--24. VLDB Endowment, 2005.
  
\bibitem{cormode2008finding}
G.~Cormode and M.~Hadjieleftheriou.
\newblock Finding frequent items in data streams.
\newblock {\em Proceedings of the VLDB Endowment}, 1(2):1530--1541, 2008.


%6
\bibitem{sigsketch}
Z.~Liu, A.~Manousis, and et~al.
\newblock One sketch to rule them all: Rethinking network flow monitoring with
  univmon.
\newblock In {\em \Proc ACM SIGCOMM}, 2016.
%7
\bibitem{asketch}
P.~Roy, A.~Khan, and G.~Alonso.
\newblock Augmented sketch: Faster and more accurate stream processing.
\newblock In {\em \Proc ACM SIGMOD}, 2016.
%8
\bibitem{icde09fcm}
D.~Thomas, R.~Bordawekar, and et~al.
\newblock On efficient query processing of stream counts on the cell processor.
\newblock In {\em \Proc IEEE ICDE}, 2009.
%9
\bibitem{durme2009streaming}
B.~V. Durme and A.~Lall.
\newblock Streaming pointwise mutual information.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  1892--1900, 2009.
%10
\bibitem{goyalIII}
A.~Goyal and H.~Daum{\'e}~III.
\newblock Approximate scalable bounded space sketch for large data nlp.
\newblock In {\em \Proc EMNLP}, 2011.
%11
\bibitem{li1sketch}
P.~Li, K.~W. Church, and T.~J. Hastie.
\newblock One sketch for all: Theory and application of conditional random
  sampling.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  953--960, 2009.
%12
\bibitem{gilbert2007one}
A.~C. Gilbert, M.~J. Strauss, J.~A. Tropp, and R.~Vershynin.
\newblock One sketch for all: fast algorithms for compressed sensing.
\newblock In {\em Proceedings of ACM symposium on Theory of computing}, 2007.

%13
\bibitem{zhang2004online}
Y.~Zhang, S.~Singh, S.~Sen, N.~Duffield, and C.~Lund.
\newblock Online identification of hierarchical heavy hitters: algorithms,
  evaluation, and applications.
\newblock In {\em \Proc ACM IMC}, 2004.

%14
\bibitem{callegari2009statistical}
C.~Callegari and N.~Cyprus.
\newblock Statistical approaches for network anomaly detection.
\newblock In {\em \Proc ICIMP}, 2009.
%15
\bibitem{zhao2006finding}
Q.~G. Zhao, M.~Ogihara, H.~Wang, and J.~J. Xu.
\newblock Finding global icebergs over distributed data sets.
\newblock In {\em \Proc ACM PODS}. ACM, 2006.

%16
\bibitem{lossyAAAI}
A.~Goyal and H.~Daum{\'e}~III.
\newblock Lossy conservative update (lcu) sketch: Succinct approximate count
  storage.
\newblock In {\em AAAI}, 2011.
%17
\bibitem{probacounting}
B.~Van~Durme and A.~Lall.
\newblock Probabilistic counting with randomized storage.
\newblock In {\em IJCAI}, pages 1574--1579, 2009.
%18
\bibitem{smoothedBF}
D.~Talbot and M.~Osborne.
\newblock Smoothed bloom filter language models: Tera-scale lms on the cheap.
\newblock In {\em EMNLP-CoNLL}, pages 468--476, 2007.

%19
\bibitem{countsketch}
M.~Charikar, K.~Chen, and M.~Farach-Colton.
\newblock Finding frequent items in data streams.
\newblock In {\em Automata, Languages and Programming}. Springer, 2002.
%20
\bibitem{cmsketch}
G.~Cormode and S.~Muthukrishnan.
\newblock An improved data stream summary: the count-min sketch and its
  applications.
\newblock {\em Journal of Algorithms}, 55(1):58--75, 2005.
%21
\bibitem{cusketch}
C.~Estan and G.~Varghese.
\newblock New directions in traffic measurement and accounting.
\newblock {\em ACM SIGMCOMM CCR}, 32(4), 2002.
%22
\bibitem{cmlog}
G.~Pitel and G.~Fouquier.
\newblock Count-min-log sketch: Approximately counting with approximate
  counters.
\newblock {\em arXiv preprint arXiv:1502.04885}, 2015.
\bibitem{sketchtheorysigmod}
F.~Rusu and A.~Dobra.
\newblock Statistical analysis of sketch estimators.
\newblock In {\em Proceedings of the 2007 ACM SIGMOD international conference
  on Management of data}, pages 187--198. ACM, 2007.
%24
\bibitem{sketchtheorytods}
F.~Rusu and A.~Dobra.
\newblock Sketches for size of join estimation.
\newblock {\em ACM Transactions on Database Systems (TODS)}, 33(3):15, 2008.
%27
\bibitem{spectralBF}
S.~Cohen and Y.~Matias.
\newblock {S}pectral bloom filters.
\newblock In {\em \Proc ACM SIGMOD}, pages 241--252, 2003.
%26
\bibitem{dynamicCF}
J.~Aguilar-Saborit, P.~Trancoso, V.~Muntes-Mulero, and J.-L. Larriba-Pey.
\newblock Dynamic count filters.
\newblock {\em ACM SIGMOD Record}, pages 26--32, 2006.



% % % % % % % % % % % %
%25
\bibitem{GPU-GAMT}
Y.~Li, D.~Zhang, A.~X. Liu, and J.~Zheng.
\newblock {GAMT}: a fast and scalable ip lookup engine for gpu-based software
  routers.
\newblock In {\em \Proc IEEE/ACM ANCS}, 2013.

%
\bibitem{YCSB}
B.~F. Cooper, A.~Silberstein, and et~al.
\newblock Benchmarking cloud serving systems with {YCSB}.
\newblock In {\em \Proc ACM SOCC}, 2010.
%
\bibitem{BF1970}
B.~H. Bloom.
\newblock Space/time trade-offs in hash coding with allowable errors.
\newblock {\em Communications of the ACM}, 13(7):422--426, 1970.
%
\bibitem{CUDA-Best}
NVIDIA Corporation.
\newblock {\em NVIDIA CUDA C Best Practices Guide, Version 5.0}, Oct. 2012.



\bibitem{zipf}
D.~M. Powers.
\newblock Applications and explanations of {Zipf}'s law.
\newblock In {\em \Proc EMNLP-CoNLL}. Association for Computational
  Linguistics, 1998.









\bibitem{GPU-NDN}
Y.~Wang, Y.~Zu, and et~al.
\newblock Wire speed name lookup: A gpu-based approach.
\newblock In {\em \Proc USENIX NSDI}, pages 199--212, 2013.




\bibitem{memcached}
{M}emcached - a distributed memory object caching system.
\newblock \url{http://memcached.org}.

\end{thebibliography}

